SCAI-QReCC Shared Task on Conversational Question Answering

Search-Oriented Conversational AI (SCAI) is an established venue that regularly puts a spotlight upon the recent work advancing the field of conversational search. SCAI'21 was organised as an independent on-line event and featured a shared task on conversational question answering. Since all of the participant teams experimented with answer generation models for this task, we identified evaluation of answer correctness in this settings as the major challenge and a current research gap. Alongside the automatic evaluation, we conducted two crowdsourcing experiments to collect annotations for answer plausibility and faithfulness. As a result of this shared task, the original conversational QA dataset used for evaluation was further extended with alternative correct answers produced by the participant systems.

==> related_work.tex <==
\section{Related Work}
\label{related_work}

\subsection{QA evaluation}

\cite{risch2021semantic} proposed SAS metric for measuring answer similarity.

\subsection{QA datasets}


